Dense Dynamic Scene Reconstruction and Camera Pose Estimation from Multi-View Videos

We address the challenging problem of dense dynamic scene reconstruction and camera pose estimation from multiple freely moving cameras -- a setting that arises naturally when multiple observers capture a shared event. Prior approaches either handle only single-camera input or require rigidly mounted, pre-calibrated camera rigs, limiting their practical applicability. We propose a two-stage optimization framework that decouples the task into robust camera tracking and dense depth refinement. In the first stage, we extend single-camera visual SLAM to the multi-camera setting by constructing a spatiotemporal connection graph that exploits both intra-camera temporal continuity and inter-camera spatial overlap, enabling consistent scale and robust tracking. To ensure robustness under limited overlap, we introduce a wide-baseline initialization strategy using feed-forward reconstruction models. In the second stage, we refine depth and camera poses by optimizing dense inter- and intra-camera consistency using wide-baseline optical flow. Additionally, we introduce MultiCamRobolab, a new real-world dataset with ground-truth poses from a motion capture system. Finally, we demonstrate that our method significantly outperforms state-of-the-art feed-forward models on both synthetic and real-world benchmarks, while requiring less memory.

==> figures/fig_ablation_initialization_noise.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=0.95\linewidth,
            height=0.55\linewidth,
            xlabel={Initialization translation noise [m]},
            ylabel={ATE Mean [m]},
            xmin=0, xmax=0.32,
            ymin=0, ymax=0.22,
            xtick={0.02, 0.05, 0.10, 0.15, 0.20, 0.30}, 
            ytick={0.00, 0.05, 0.10, 0.15, 0.20},
            xticklabel style={/pgf/number format/fixed, /pgf/number format/fixed zerofill, /pgf/number format/precision=2, font=\footnotesize},
            yticklabel style={/pgf/number format/fixed, /pgf/number format/fixed zerofill, /pgf/number format/precision=2, font=\footnotesize},
            xlabel style={font=\small},
            ylabel style={font=\small},
            grid=both,
            grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt, draw=gray!30},
            tick align=outside,
        ]
        
        \pgfplotsset{bsl/.style={dashed, line width=0.6pt}}
        
        \addplot[bsl, violet, domain=0:0.32] {0.196} node[pos=0.20, above, font=\tiny] {CUT3R (0.196)};
            
        \addplot[bsl, brown, domain=0:0.32] {0.180} node[pos=0.20, above, font=\tiny] {Fast3R (0.180)};
            
        \addplot[bsl, red, domain=0:0.32] {0.143} node[pos=0.20, above, font=\tiny] {$\texttt{w/o}$ \hyperref[para:init]{W.B. Init.} (0.143)};
            
        \addplot[bsl, orange, domain=0:0.32] {0.133} node[pos=0.20, below, font=\tiny] {COLMAP (0.133)};
            
        \addplot[bsl, gray, domain=0:0.32] {0.020} node[pos=0.20, above, font=\tiny] {FastVGGT (0.020)};

        \addplot[
            color=blue,
            mark=*,
            line width=1.5pt,
            mark size=2pt,
            nodes near coords,
            every node near coord/.append style={
                font=\tiny, 
                anchor=south east,
                xshift=-2pt,
                /pgf/number format/fixed,
                /pgf/number format/fixed zerofill,
                /pgf/number format/precision=2
            }
        ] coordinates {
            (0.02, 0.0164)
            (0.05, 0.0404)
            (0.10, 0.0443)
            (0.15, 0.1084)
            (0.20, 0.1284)
            (0.30, 0.1594)
        };
        
        \end{axis}
    \end{tikzpicture}
    \caption{\textbf{Robustness to initialization translation noise.} 
    The X-axis shows the translation noise added to the initialization poses, and the Y-axis shows the final evaluated ATE.
    Under small perturbation noise, our method can still maintain good results (under 0.1m).
    When the noise is large, for example, with 0.15m noise, the trajectory degrades much.
    The result shows that our method can recover from imperfectly initialized poses under mild noisy poses.
    }
    \label{fig:init_noise_comparison}
\end{figure}

==> sec/0_abstract.tex <==
\begin{abstract}
% Problem statement
We address the problem of dense dynamic scene reconstruction from multiple time-synchronized, freely moving cameras---a setting that arises naturally when multiple observers capture a shared event but lacks support from existing methods.
% Previous work
Prior approaches either handle only single-camera input or require rigidly mounted, pre-calibrated camera rigs, limiting their practical applicability.
% Our method
We propose a two-stage optimization framework that jointly estimates camera poses and dense per-frame depth across all cameras.
In the first stage, we extend single-camera visual SLAM to the multi-camera setting by constructing a spatiotemporal connection graph that exploits both intra-camera temporal continuity and inter-camera spatial overlap, enabling consistent scale and robust tracking.
In the second stage, we refine depth and camera poses by optimizing dense inter- and intra-camera consistency using wide-baseline optical flow.
% Results
We introduce MultiCamRobolab, a new real-world dataset with ground-truth poses from a motion capture system, and demonstrate that our method significantly outperforms state-of-the-art feedforward models on both synthetic and real-world benchmarks while requiring less memory.
\end{abstract}


==> sec/5_limitation.tex <==
\section{Limitation}
Though performing better than baselines, we found some limitations during our experiments.
When the two cameras are facing each other and then move in parallel,  no overlap can be found in this case. 
Even though the VGGT can robustly recover the initial scene, the tracking might not remain consistent and accurate due to the lack of inter-camera connections.
This problem can be alleviated by adding more cameras, which will bring more connections across different cameras.
We can also utilize the ability of a robust feed-forward model (like VGGT) to get pose prediction in the low overlap case.
The tracking quality for all methods is better on RoboArm than on RoboDog, because in the RoboArm scene, the two cameras always have a relatively large overlap. 

==> tables/3_camera_tracking.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\caption{
\color{red}{To add captions}
}
\resizebox{0.3\textwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Method} 
    & ATE$\downarrow$ & RTE$\downarrow$ & RRE$\downarrow$ \\
    \midrule
    COLMAP~\cite{schonberger2016structure}
    & 0.343 & 0.013 & 0.376\\
    \hdashline
    Fast3R~\cite{yang2025fast3r}
    & 0.376 & 0.154 & 1.825\\
    FastVGGT~\cite{shen2025fastvggt}
    & 0.032 & 0.017 & 0.363 \\
    CUT3R~\cite{wang2025continuous}
    & 0.474 & 0.0351 & 0.467\\
    \hdashline
    Ours
    & 0.020 & 0.011 & 0.326\\
    \bottomrule
    \end{tabular}
}
\label{tab:robotracking_robodog}
\end{table}

==> tables/multiplecam_robolab_pose_full.tex <==
% TODO: improve the format!

\begin{table}[t]
\centering
\caption{Quantitative tracking evaluation on the RoboLab Dataset. Lower is better for all metrics; $\dagger$: To avoid memory overflow when using Fast3R with all frames, we process every second frame as input for Fast3R.}
\label{tab:robolab_tracking}
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Scenes}} 
& \multicolumn{3}{c}{\textbf{Fast3R}$^\dagger$~\cite{yang2025fast3r}} 
& \multicolumn{3}{c}{\textbf{CUT3R}~\cite{wang2025continuous}}
& \multicolumn{3}{c}{\textbf{Ours}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 
 & ATE$\downarrow$ & RTE$\downarrow$ & RPE$\downarrow$ 
 & ATE$\downarrow$ & RTE$\downarrow$ & RPE$\downarrow$ 
 & ATE$\downarrow$ & RTE$\downarrow$ & RPE$\downarrow$ \\
\midrule
$\texttt{Robodog01}$ &0.049  &0.052  &1.166  &0.096  &0.008  &0.243  &0.011  &0.005  &0.185  \\
$\texttt{Robodog02}$ &0.053  &0.053  &0.965  &0.125  &0.007  &0.189  &0.008  &0.003  &0.139  \\
$\texttt{Robodog03}$ &0.440  &0.094  &2.636  &0.433  &0.022  &0.306  &0.242  &0.005  &0.130  \\
$\texttt{Robodog04}$ &0.101  &0.078  &1.186  &0.255  &0.017  &0.329  &0.012 &0.002  &0.176  \\
$\texttt{RoboArm01}$ &0.037  &0.041  &1.150  &0.053  &0.002  &0.101  &0.004 &0.001  &0.050  \\
$\texttt{RoboArm02}$ &0.068  &0.059  &0.615  &0.047  &0.003  &0.097  &0.004  &0.0008  &0.139  \\
$\texttt{RoboArm03}$ &0.060  &0.066  &1.373  &0.037  &0.004  &0.097  &0.008  &0.001  &0.076  \\
$\texttt{RoboArm04}$ &0.027  &0.031  &0.540  &0.083  &0.004  &0.122  &0.004  &0.002  & 0.176 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/mvv_traj_qualtative.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/qualtative_mvv.jpg}
    \hfill
    % \includegraphics[width=0.45\linewidth]{figures/mvv_img.jpg}
    \caption{Visualization of estimated trajectories on one of the MultiCamVideo scenes.
    Our method achieves almost fully aligned trajectories with the ground truth.
    Although CUT3R is designed for dynamic videos, it cannot recover an accurate trajectory from any single video here.}
    \label{fig:mvv_qual_traj}
\end{figure}


==> tables/robolab_scene_consitency.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|c|c}
\toprule
\textbf{Method} & 
\textbf{RoboDog} &
\textbf{RoboArm} \\
\cmidrule(lr){2-3}
& MSE$\downarrow$ & MSE$\downarrow$ \\
\midrule
Fast3R~\cite{yang2025fast3r} & 1.058 & 0.446 \\
CUT3R~\cite{wang2025continuous} & 0.595 & 0.340 \\
Ours & 0.200 & 0.127 \\
\bottomrule
\end{tabular}
\caption{Scene consistency evaluation on the self-collected RoboLab datasets.}
\label{tab:scene_consistency_comp}
\end{table}


==> tables/robolab_video_depth.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & 
\multicolumn{2}{c|}{\textbf{RoboDog}} &
\multicolumn{2}{c|}{\textbf{RoboArm}} &
\multicolumn{2}{c}{\textbf{DynamicHuman}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
&Abs Rel$\downarrow$ & $\delta_{1.25}$ $\uparrow$ & Abs Rel$\downarrow$ & $\delta_{1.25}$ $\uparrow$ & Abs Rel$\downarrow$ & $\delta_{1.25}$ $\uparrow$ \\
\midrule
CUT3R~\cite{wang2025continuous} & & & &  & \\
Ours & & & & & &  \\
\bottomrule
\end{tabular}
\caption{Video depth evaluation on the self-collected RoboLab datasets.}
\label{tab:comparison}
\end{table*}

